Simple and Principled Uncertainty Estimation with Deterministic Deep Learning via Distance Awareness

Bayesian neural networks (BNN) and deep ensembles are principled approaches to estimate the predictive uncertainty of a deep learning model. However their practicality in real-time, industrial-scale applications are limited due to their heavy memory and inference cost. This motivates us to study principled approaches to high-quality uncertainty estimation that require only a single deep neural network (DNN). By formalizing the uncertainty quantification as a minimax learning problem, we first identify input distance awareness, i.e., the model's ability to quantify the distance of a testing example from the training data in the input space, as a necessary condition for a DNN to achieve high-quality (i.e., minimax optimal) uncertainty estimation. We then propose Spectral-normalized Neural Gaussian Process (SNGP), a simple method that improves the distance-awareness ability of modern DNNs, by adding a weight normalization step during training and replacing the output layer with a Gaussian process. On a suite of vision and language understanding tasks and on modern architectures (Wide-ResNet and BERT), SNGP is competitive with deep ensembles in prediction, calibration and out-of-domain detection, and outperforms the other single-model approaches.

==> preamble/packages.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts

\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{wrapfig}

% Use fancyhdr package
\RequirePackage{multicol}
\RequirePackage{fancyhdr}
\RequirePackage{color}
\RequirePackage{algorithm}
\RequirePackage{algorithmic}
%\usepackage{algorithm}
%\usepackage{algorithmicx}
%\usepackage{algpseudocode}
%\RequirePackage{natbib}
\RequirePackage{eso-pic} % used by \AddToShipoutPicture 
\RequirePackage{forloop}

% Recommended, but optional, packages for figures and better typesetting:
\usepackage[numbers]{natbib}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage[font=footnotesize]{caption}
\usepackage{subcaption}
\usepackage{booktabs} % for professional tables

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{mathptmx}
\usepackage{soul}

%\usepackage{lipsum}

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2019} with \usepackage[nohyperref]{icml2019} above.
%\usepackage{color}
\usepackage[dvipsnames]{xcolor}
\definecolor{mydarkblue}{rgb}{0,0.08,0.45}
\usepackage[colorlinks,citecolor=mydarkblue,urlcolor=mydarkblue,linkcolor=mydarkblue
]{hyperref}
%\usepackage{hyperref}
\usepackage{comment}
\usepackage[hang,flushmargin]{footmisc}
      % hyperlinks
\usepackage{url}
% 
\def\UrlBreaks{\do\/\do-}
%\usepackage{breakurl}% simple URL typesetting
%

% Attempt to make hyperref and algorithmic work together better:
%\newcommand{\theHalgorithm}{\arabic{algorithm}}

% use glossary
\usepackage
[acronym,nowarn,section,nonumberlist]{glossaries}
\glsdisablehyper{}

% import external document
\usepackage{xr}



% theorem
\usepackage{amsthm}

% custom toc
\usepackage[page,header]{appendix}
\usepackage{titletoc}
\usepackage{etoc}

\usepackage{"./macro/GrandMacros"}
\usepackage{"./macro/Macro_BIO235"}


==> section/experiment-icml.tex <==
In this section, we perform an extensive assessment of the properties of the uncertainty estimates obtained from \gls{SNGP}. 
\vspace{-0.5em}
\subsection{2D Synthetic Benchmark}
\label{sec:exp_2d}
%\vspace{-0.5em}

We first study the behavior of the uncertainty surface of a \gls{SNGP} model under a suite of 2D classification benchmarks. 
%Our goals are to (1) illustrate the role of the \textit{input distance awareness} property in a model's ability in uncertainty quantification, and (2) to understand the effect of the two proposed model components (i.e., the bi-Lipschitz constraint and the \gls{GP} layer) on a deep model's  \textit{input distance awareness} property. 
Specifically, we consider the \textit{two ovals} benchmark (Figure \ref{fig:2d_exp}, row 1) and the \textit{two moons} benchmark (Figure \ref{fig:2d_exp}, row 2). The \textit{two ovals} benchmark consists of two near-flat Gaussian distributions, which represent the two in-domain classes (orange and blue) that are separable by a linear decision boundary. There also exists an \gls{OOD} distribution (red) that the model doesn't observe during training. Similarly, the \textit{two moons} dataset consists of two banana-shaped distributions separable by a nonlinear decision boundary. We consider a 12-layer, 128-unit deep architecture ResFFN-12-128. The full experiment details are in Appendix \ref{sec:exp_detail}.
\input{"./section/figures/2d_exp_moon_icml"} % ICML

Figure \ref{fig:2d_exp} shows the results, where the  background color visualizes the uncertainty surface output by each model. We first notice that the shallow Gaussian process models (Figures \ref{fig:2d_exp_oval_gp} and \ref{fig:2d_exp_moon_gp})  exhibit an expected behavior for high-quality predictive uncertainty: 
it generates low uncertainty in $\Xsc_{\texttt{IND}}$ that is supported by the training data (purple color), and generates high uncertainty when $\bx$ is far from $\Xsc_{\texttt{IND}}$ (yellow color), i.e., \textit{input distance awareness}. As a result, the shallow \gls{GP} model is able to assign low confidence to the \gls{OOD} data (colored in red), indicating reliable uncertainty quantification. On the other hand, deep ensembles (Figures \ref{fig:2d_exp_oval_deepens},  \ref{fig:2d_exp_moon_deepens}) %and MC Dropout (Figures \ref{fig:2d_exp_oval_mc}, \ref{fig:2d_exp_moon_mc}) 
are based on dense output layers that are not distance aware. As a result, %both methods 
they quantify their predictive uncertainty based on the distance from the decision boundaries, assigning low uncertainty to \gls{OOD} examples even if they are far from the data.
Finally, the DNN-GP (Figures \ref{fig:2d_exp_oval_deepgp} and\ref{fig:2d_exp_moon_deepgp}) and \gls{SNGP} (Figures \ref{fig:2d_exp_oval_sngp} and\ref{fig:2d_exp_moon_sngp}) both use \gls{GP} as their output layers, but with \gls{SNGP} additionally imposing the spectral normalization on its hidden mapping $h(.)$. As a result, the DNN-GP's uncertainty surfaces are still strongly impacted by the distance from decision boundary, likely caused by the fact that the un-regularized hidden mapping $h(\bx)$ is free to discard information that is not relevant for prediction. On the other hand, the \gls{SNGP} is able to maintain the \textit{input distance awareness} property via its bi-Lipschitz constraint, and exhibits a uncertainty surface that is analogous to the gold-standard model (shallow \gls{GP}) despite the fact that \gls{SNGP} is based on a 12-layer network.

\vspace{-0.5em}

\subsection{Vision and Language Understanding}
\label{sec:exp_ml}
%\vspace{-0.5em}
%In this section, we quantitatively evaluate the method's performance in prediction, calibration and out-of-domain detection across both vision and language modalities. 
%\tbw{I'm missing training times for the different methods.  Is there a way to get those?  Part of the argument made in the paper is also that we're making contributions in training speedup.} 
%\tbw{Consider shortening since you're going to go through the experimental results next.  In fact, you can probably just fold in some of the details in the narrative of each of the two sections (vision and language).}
%We consider two practical modern architectures: Wide ResNet-28-10 \citep{zagoruyko_wide_2017} and BERT \citep{devlin_bert:_2018}. We benchmark \gls{SNGP} against a deterministic baseline and two popular ensemble approaches: \gls{MCD} (with 10 dropout samples) and deep ensembles (with 10 models), all trained with models with no spectral regularization and dense output layer. We also consider two recently proposed \gls{GP} and \gls{RBF}-based single-model approaches that focus on uncertainty quantification: \gls{MCDGP} which applies 10-sample \gls{MCD} to a deep model with \gls{RFF}-based output layer\citep{tran_calibrating_2019}, and 
%\gls{DUQ} which applies a two-sided gradient penalty to a deep model with a \gls{RBF}-based output layer \citep{van_amersfoort_simple_2020}. \gls{SNGP} differs from these two approaches in the method for regularizing neural network mapping (spectral normalization), and the method for estimating the predictive uncertainty (closed-form covariance update (\ref{eq:gp_posterior})). In both vision and language experiments, the single-model \gls{SNGP} is competitive in performance with that of a 10-model deep ensemble, and outperforms the other approaches.

\paragraph{CIFAR-10 and CIFAR-100}
\label{sec:cifar}
%\tbw{if you elided the rest of the intro of this section, I'd say something like this which blends the first and second paragraphs: We fist evaluation \gls{SNGP} on a wide ResNet-28-10 against a deterministic baseline and two ensemble approaches: \gls{MCD} (with 10 dropout samples) and Deep ensembles (with 10 models), all trained with models with no spectral regularization and dense output layer. We evaluate the model's predictive accuracy and calibration error under both clean and corrupted version of the CIFAR-10 and CIFAR-100 testing data.  The corrupted data, ... }
We first evaluate \gls{SNGP} on a Wide ResNet 28-10 \citep{zagoruyko_wide_2017} against a deterministic baseline and two ensemble approaches: \textbf{\gls{MCD}} (with 10 dropout samples) and \textbf{deep ensembles} (with 10 models), all trained with a dense output layer and no spectral regularization. We also consider two single-model approaches: \gls{MCDGP} (with 10 samples) and \gls{DUQ} (see Section \ref{sec:related}). 
%\gls{SNGP} differs from these two approaches in its regularization method for the hidden mapping (spectral normalization), and its method for estimating predictive uncertainty (closed-form predictive variance (\ref{eq:gp_posterior})). 
We evaluate the model's predictive accuracy and calibration error under both clean CIFAR testing data and its corrupted versions termed CIFAR-C \citep{hendrycks_benchmarking_2018}. To evaluate the model's \gls{OOD} detection performance, we consider a  standard \gls{OOD} task using \glsunset{SVHN}\gls{SVHN} as the \gls{OOD} dataset for a model trained on CIFAR-10/-100, and a difficult \gls{OOD} task using CIFAR-100 as the \gls{OOD} dataset for a model trained on CIFAR-10, and vice versa. Full experiment details and additional results are in Appendix \ref{sec:exp_detail}. 
\input{./section/tables/cifar}
%\input{./section/tables/cifar10}
%\input{./section/tables/cifar100}
Table \ref{tb:cifar} reports the results. As shown, for predictive accuracy, \gls{SNGP} is competitive with that of a deterministic network, and outperforms the other single-model approaches. For calibration error, \gls{SNGP} clearly outperform the other single-model approaches and is competitive with the deep ensemble. Finally, for \gls{OOD} detection, \gls{SNGP} outperforms not only the deep ensembles and \gls{MCD} approaches that are based on a dense output layer, but also the \gls{MCDGP} and \gls{DUQ} that are based on the \gls{GP} layer, illustrating the importance of the \textit{input distance awareness} property for high-quality performance in uncertainty quantification.
%\imp{\textbf{Dustin}:SNGP seems to perform worse on accuracy and ECE on in- and OOD, but perform better on AUC-PR for SVHN and CIFAR-100. Do you have any intuitions or ablations that dig into this?}
%\imp{\textbf{Dustin}:Where does BatchEnsemble or rank-1 BNNs compare as baselines here?}
\paragraph{Detecting Out-of-Scope Intent in Conversational Language Understanding}
\label{sec:clinc}

To validate the method beyond image modalities, we also evaluate \gls{SNGP} on a practical language understanding task where uncertainty quantification is of natural importance: dialog intent detection \citep{larson_evaluation_2019, vedula_towards_2019, yaghoub-zadeh-fard_user_2020, zheng_out--domain_2020}.
In a goal-oriented dialog system (e.g. chatbot) built for a collection of in-domain services, it is important for the model to understand if an input natural utterance from an user is in-scope (so it can activate one of the in-domain services) or out-of-scope (where the model should abstain). To this end, we consider training an intent understanding model using the CLINC \gls{OOS} intent detection benchmark dataset \citep{larson_evaluation_2019}. Briefly, the \gls{OOS} dataset contains data for 150 in-domain services with 150 training sentences in each domain, and also 1500 natural out-of-domain utterances. We consider the BERT$_{\texttt{Base}}$ architecture, which is a 12-layer transformer pre-trained on a large language corpus \citep{devlin_bert:_2018}. We train the models only on in-domain data, and evaluate their predictive accuracy on the in-domain test data, their calibration and \gls{OOD} detection performance on the combined in-domain and out-of-domain data. The results are in Table \ref{tb:clinc}. As shown, consistent with the previous vision experiments, \gls{SNGP} is competitive in predictive accuracy when compared to a deterministic baseline, and outperforms other approaches in calibration and \gls{OOD} detection.

\input{./section/tables/clinc}

==> section/figures/2d_exp_moon_icml.tex <==
\begin{figure}[th!]
    \centering
    \subcaptionbox{GP\label{fig:2d_exp_oval_gp}}{
    \includegraphics[width=0.2\columnwidth]{./figures/2d/oval_gp}}
    \subcaptionbox{DE\label{fig:2d_exp_oval_deepens}}{
    \includegraphics[width=0.2\columnwidth]{./figures/2d/oval_deep_ens}}
   % \subcaptionbox{MC Dropout\label{fig:2d_exp_oval_mc}}{
   % \includegraphics[width=0.18\columnwidth]{./figures/2d/oval_mc}}
    \subcaptionbox{DNN-GP \label{fig:2d_exp_oval_deepgp}}{
    \includegraphics[width=0.2\columnwidth]{./figures/2d/oval_deep_gp}}
    \subcaptionbox{\gls{SNGP} (ours) \label{fig:2d_exp_oval_sngp}}{
    \includegraphics[width=0.25\columnwidth]{./figures/2d/oval_sngp}}

    \subcaptionbox{GP\label{fig:2d_exp_moon_gp}}{
    \includegraphics[width=0.2\columnwidth]{./figures/2d/moon_gp}}
    \subcaptionbox{DE\label{fig:2d_exp_moon_deepens}}{
    \includegraphics[width=0.2\columnwidth]{./figures/2d/moon_deep_ens}}
   % \subcaptionbox{MC Dropout\label{fig:2d_exp_moon_mc}}{
   % \includegraphics[width=0.18\columnwidth]{./figures/2d/moon_mc}}
    \subcaptionbox{DNN-GP \label{fig:2d_exp_moon_deepgp}}{
    \includegraphics[width=0.2\columnwidth]{./figures/2d/moon_deep_gp}}
    \subcaptionbox{\gls{SNGP} (ours)  \label{fig:2d_exp_moon_sngp}}{
    \includegraphics[width=0.25\columnwidth]{./figures/2d/moon_sngp}}
   \vspace{-0.5em}
    \caption{
    \small{Uncertainty surfaces of \gls{GP},  DNN approaches such as deep ensembles (DE) and DNN-GP, and our method SNGP.
   % The uncertainty surface of a \gls{GP} and  DNN approaches such as deep ensembles (DE) and DNN-GP on the \textit{two ovals} (Top Row) and \textit{two moons} (Bottom Row) 2D classification benchmarks. Our method SNGP is the only \gls{DNN}-based approach achieving a distance-aware uncertainty similar to the gold-standard \gls{GP}.  Training data for positive (\textbf{Orange}) and negative classes (\textbf{Blue}) . OOD data (\textbf{Red}) not observed during training. Background color represents the  estimated model uncertainty (See \ref{fig:2d_exp_oval_sngp} and \ref{fig:2d_exp_moon_sngp} for color map).
    %See Section 5.1 for details.
    }}
     \vspace{-0.5em}
    \label{fig:2d_exp}
\end{figure}

==> section/figures/schematic.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.85\columnwidth]{./figures/idea}
    \caption{A schematic of the proposed \textit{\glsfirst{SNGP}} approach}
    \label{fig:sngp_idea}
\end{figure}


==> section/proof/calib_error.tex <==
\section{Accurate $p^*(y|\bx)$ Approximation implies Low Calibration Error}
\label{sec:l1_implies_ece}

Recall the definition of the calibration error:
\begin{align*}
\mathbb{E}_{\Dsc}
    \Big[\Big| \bbP(y=\hat{y} | \hat{p} = p ) - p \Big| \Big],
\end{align*}
where $\hat{p} = p(\hat{y}|\bx)$. Also note that in sufficiently large sample, $ \bbP(y=\hat{y} | \hat{p} = p )$ converges to an expectation of the data-generation distribution $p^*$ by the weak law of large numbers:
\begin{align*}
\bbP(y=\hat{y} | \hat{p} = p ) \stackrel{P}{\rightarrow}
\mathbb{E}_{\bx: p(\hat{y}|\bx)=p}\Big[  p^*(\hat{y}|\bx) \Big].
\end{align*}
Therefore by the continuous mapping theorem, we can rewrite the definition of calibration error as:
\begin{alignat*}{3}
\mathbb{E}_{\Dsc}
    \Big[\Big| \bbP(y=\hat{y} | \hat{p} = p ) - p \Big| \Big]
    &\stackrel{P}{\rightarrow}
    \mathbb{E}_{\Dsc}
    \Big[\Big| \mathbb{E}_{\bx: p(\hat{y}|\bx) = p} 
    \big[ p^*(\hat{y} \big|\bx )\big] - p \Big| \Big]\\
    &=
    \mathbb{E}_{\Dsc}
    \Big[\Big| \mathbb{E}_{\bx: p(\hat{y}|\bx) = p} 
    \big[ p^*(\hat{y} \big|\bx )  - p \big] \Big| \Big] 
    \qquad\quad &&\mbox{(move $p$ inside expectation)}
    \\
    &=
    \mathbb{E}_{\Dsc}
    \Big[\Big| \mathbb{E}_{\bx: p(\hat{y}|\bx) = p} 
    \big[ p^*(\hat{y} \big|\bx )  - p(\hat{y}|\bx) \big] \Big| \Big]
    \qquad\quad &&\mbox{(use the fact $p(\hat{y}|\bx) = p$)}
    \\
    &\leq
    \mathbb{E}_{\Dsc}\mathbb{E}_{\bx: p(\hat{y}|\bx) = p}
    \Big[ \Big| 
     p^*(\hat{y} \big|\bx )  - p(\hat{y}|\bx) \Big| \Big]
    \qquad\quad &&\mbox{(Jensen's Inequality)}
    \\
    &=
    \mathbb{E}_{\Dsc}
    \Big[ \Big| 
    p^*(\hat{y} \big|\bx )  - p(\hat{y}|\bx) \Big| \Big], 
\end{alignat*}
where the last line is the empirical $L_1$ distance between data-generating distribution $p^*(\hat{y} \big|\bx )$ and model prediction $p(\hat{y}|\bx)$. 

Consequently, we have shown that in sufficiently large sample, the calibration error is upper bounded by the $L_1$ distance between $p(y|\bx)$ and $p^*(y|\bx)$, which implies that a model that can accurately approximate $p^*(y|\bx)$ is expected to have low calibration error.


==> section/section_old/background_old.tex <==
\section{Background}

\paragraph{Notation and Problem Setup}

Consider a data-generation distribution $p^*(y|\bx): \Xsc \times \Ysc \rightarrow [0, 1]$, where $\Xsc \subset \real^d$ is the domain of the input $\bx$, and $\Ysc \in [0, 1]^K$ is the space of $K$-class labels. Given data $\Dsc=\{y_i, \bx_i\}_{i=1}^N \sim p^*(y|\bx)$, a common goal of machine learning modeling is to estimate the data generation distribution using a model $p(y|\theta, \bx)$, e.g, $p(y|\theta, \bx)=Multinomial(p_k = h_W(\bx)\beta_k)$ where $f_W$ is a neural network and $\theta=(W, \{\bbeta_k\}_{k=1}^K)$. It is important to notice that both the \textit{domain} $\Xsc$ and the \textit{mapping} $p^*(y|\bx)$ are components of the data generation distribution that need to be inferred from data. As such, after learning a parameter distribution $p(\theta|\Dsc)$, a goal of the \gls{UQ} methods is to produce a predictive distribution $p(y|x) = \int p(y|\bx, \theta)p(\theta|\Dsc) d\theta$ that properly encapsulates the  uncertainties about both the mapping $p^*(y|\bx)$ and about the domain probability $p(\bx \in \Xsc)$, i.e.:
\begin{alignat*}{6}
    p(y |\bx) 
    &= p(y|\bx, \bx \in \Xsc)&& * p(\bx \in \Xsc) 
    && + p(y|\bx, \bx \not\in \Xsc)&& * p(\bx \not\in \Xsc)\\
    &= 
    \quad p_{\texttt{IND}}(y|\bx)&& * p(\bx \in \Xsc) 
    && + 
    \quad p_{\texttt{OOD}}(y|\bx)&& * p(\bx \not\in \Xsc).
\end{alignat*}
In the above, $p_{\texttt{IND}}(y|\bx) = p(y|\bx, \bx \in \Xsc)$ is the model's \gls{IND} predictive distribution. As the sample size $N$ increases, $p_{\texttt{IND}}(y|\bx)$ should converge quickly toward $p^*(y|\bx)$ such that the model's predictive probability reflects the empirical, long-running frequency of the event $y|\bx$, i.e., \textit{in-domain calibration} \citep{gneiting_probabilistic_2014}. On the other hand, $p_{\texttt{OOD}}(y|\bx) = p(y|\bx, \bx \not\in \Xsc)$ is a maximum-entropy distribution (i.e., the  discrete uniform distribution) encoding the model's \gls{OOD} uncertainty. Given a testing instance $\bx$, $p(\bx \in \Xsc)$ should meaningfully capture its distance from the domain $\Xsc$, such that the model exhibits high uncertainty in the state of lacking support from the training data, i.e., the \textit{out-of-domain generalization} \citep{lakshminarayanan_simple_2017}.

\paragraph{Conditions for High Quality \gls{UQ}}
Correspondingly, there are two \gls{UQ} metrics for assessing a model's ability in calibration and in \gls{OOD} generalization, respectively. The first metric is the \textit{calibration error}: $\mathbb{E}_{\Dsc} \Big[\Big| \bbP(y=\hat{y} | \hat{p} = p ) - p \Big| \Big]$, where $\hat{p} = p(\hat{y}|\bx)$ indicates the model's predictive probability \citep{guo_calibration_2017}. Given a probabilistic prediction $p(\hat{y}|\bx)$, calibration error assesses the correspondence between the model's predictive confidence $\hat{p}=p(\hat{y}|\bx)$ and its actual probability of being correct $\bbP(y=\hat{y} | \hat{p} = p )$.
A sufficient condition for a model to achieve low calibration error is to achieve high-quality estimation of in-domain distribution $p_{\texttt{IND}}(y|\bx)$, since the calibration error is upper bounded by the $L_1$ distance between $p_{\texttt{IND}}(y|\bx)$ and $p^*(y|\bx)$ in large sample (see Appendix \ref{sec:l1_implies_ece} for the derivation of this fact). The second metric is the \textit{out-of-domain accuracy}: given a set of mixed of \gls{IND} and \gls{OOD} samples with varying in-domain probability $p^*(\bx' \in \Xsc)$, the model is asked to build a binary \gls{OOD} classifier by filtering out testing examples whose model uncertainty exceed a certain threshold $\tau$ \citep{ovadia_can_2019}. Clearly, a sufficient condition for a model to achieve high \gls{OOD} accuracy is the reliable quantification of its out-of-domain probability $p(\bx \in \Xsc)$.

Consequently, for a deep learning model to perform well in calibration and in out-of-domain detection.


\subsection{Types of Uncertainty in Deep Learning}
\label{sec:uncertainty_types}

\subsection{A Unified View of \gls{UQ} Methods under Bayesian Principle}
\label{sec:methods_review}


==> section/section_old/bayesian.tex <==
Given data $\{y_i, \bx_i\}_{i=1}^N$, the multinomial opinion (\ref{eq:opinion}) can be learned by updating the Dirichlet distribution using Bayes' rule \citep{josang_consensus_2002, josang_probabilistic_2007}.
%To this end, Bayesian method provides a principled solution to modeling predictive  uncertainty by treating $\bp$ as a random variable and learns its distribution from data using the Bayes' rule. 
Specifically, given the \textit{a priori} multinomial opinion represented by the Dirichlet prior distribution $P_{\balpha_0}(\bp)$, the model learns the \textit{a posteriori} opinion $P(\bp|y)$ by updating the prior distribution with respect to the data likelihood $P(y|\bp)$ (\ref{eq:multinom}):
\begin{align}
    P(\bp|y) &= 
    \frac{P(y|\bp)P_{\balpha_0}(\bp)}{
    \int P(y|\bp)P_{\balpha_0}(\bp) d\bp
    }.
    \label{eq:bayes}
\end{align}

In this work, we assume $\bp$ to follow a Dirichlet distribution:
\begin{align}
    P_{\balpha_0}(\bp) \propto \prod_{k=1}^K p_k^{\alpha_{0k} - 1},
    \label{eq:dirichlet}
\end{align}
Since Dirichlet distribution is the conjugate prior for the Multinomial likelihood, the posterior distribution is known to also be a Dirichlet distribution $P_{\balpha}(\bp)$ indexed by the posterior parameters $\balpha$ \citep{gelman_bayesian_2013}. Consequently, the problem of inferring the the posterior distribution $P(\bp|y)$ is reduced to estimating the Dirichlet parameters $\balpha$, which can be learned scalably using neural networks by taking an optimization-based formulation of Bayesian inference (Section \ref{sec:idl}).


==> section/section_old/dst.tex <==
We consider a multi-class classification setting with $K$ possible classes $\Theta=\{1, \dots, K\}$. Given data $\{y, \bx\}$, the classic approach based on probability calculus is to learn a probability vector $\bp=[p_1, \dots, p_K]$, where $p_k$ is a \gls{PMF}  that maps each class label $k \in \Theta$ to a value between $[0, 1]$, i.e.,
\begin{align*}
    p_k = P(y = k), \quad \sum_{k=1}^K p_k = 1,
\end{align*}
which represents the model's degree of belief that the instance $\bx$ belongs to the $k^{th}$ category.

In the context of machine learning, $\bp$ is often parametrized as the softmax transformation of a multi-output neural network $f=[f_1, \dots, f_K]$, i.e., $p_k = softmax(f_k(\bx))$. Given data, model training is performed by learning the neural network $\hat{f}$ that minimizes the cross-entropy loss, i.e., the negative log-likelihood of the multinomial distribution:
\begin{align}
P(y|\bp) &\propto \prod_{k=1}^K p_k^{y_k}.\label{eq:multinom}
%\\
%\Lsc_{CE}(f) &= -\sum_{k=1}^K y_k * log \big(p_k\big),
%\label{eq:ce_loss}
\end{align}
and prediction is performed by computing the predicted class probabilities $\hat{\bp} = softmax\big(\hat{f}(\bx)\big)$ using the trained network $\hat{f}$.

A disadvantage of this classic approach is the model's lack of ability in communicating its predictive uncertainty, i.e., 
whether the model believes that there is sufficient evidence in the training data to support its conclusion about the prediction $\hat{\bp}(\bx)$. For example, when predicting the outcome of a coin toss (i.e., head or tail), regardless of whether it observed millions of tosses $\{head=10^6, tail=10^6\}$ or just two tosses $\{head=1, tail=1\}$, the model will always output the same distribution $\hat{\bp}=[0.5, 0.5]$, failing to communicate the fact that its prediction is much less confident (and likely less trustworthy) when observing only two tosses.

To this end, the \gls{DST} provides a principled solution for quantifying model uncertainty. 
%In the context of multi-class classification, \gls{DST} effectively creates a $(K+1)^{th}$ category representing "I don't know". 
\gls{DST} generalizes the probability calculus by replacing the probability function $P(.)$ with a \textit{mass function} $m(.)$. %Like the probability function, the belief function $m(.)$ assigns non-negative mass to components of $Y$ that adds up to 1; but
Unlike the probability function, the belief function can assign unique positive mass to any subset of $Y$, rather than just its  singletons $y_k$ (i.e., the class labels). As a result, we can express model belief for the $k^{th}$ category as a mass assignment to the singleton $y_k$, i.e., $b_k = m(y=k)$, and express model uncertainty as the mass assignment to the full set $u = m(y \in \Theta)$, which represents the model's inclination to not claim any specific knowledge about $y$ beyond the fact that it is a member of $\Theta$. This gives rise to the below \textit{\gls{bba}}:
\begin{align}
    b_k = m(y = k),\, u = m(y \in \Theta),\; \sum_{k=1}^K b_k + u = 1,
    \label{eq:bba}
\end{align}
where we term $b_k$ the \textit{belief mass} for the $k^{th}$ category, and $u$ the \textit{uncertainty mass} for the overall prediction. In the context of multi-class classification, this effectively gives rise to the $(K+1)^{th}$ category representing ``I don't know".

The next question is how to learn such belief and uncertainty assignment from data. To this end, we notice that the belief assignment in (\ref{eq:bba}) is known as the \textit{Dirichlet \gls{bba}} in the \gls{DST} literature, whose update mechanism bears a strong connection with the familiar Bayesian learning for an Multinomial-Dirichlet model \citep{josang_consensus_2002, josang_probabilistic_2007}. Specifically, every Dirichlet \gls{bba} can be represented by a Dirichlet distribution for $K$ categories:
\begin{align}
    P_{\balpha}(\bp) \propto \prod_{k=1}^K p_k^{\alpha_{k} - 1},
    \label{eq:dirichlet}
\end{align}
where $\alpha_{k} \geq 1$ are the \textit{concentration parameters} of the Dirichlet distribution. 
In the \gls{DST} nomenclature, this Dirichlet distribution $P_{\balpha}(\bp)$ represents the model's subjective opinion about the multinomial probability assignment $\bp$, i.e., a \textit{multinomial opinion}. $\alpha_k$ represents the strength of evidence for the $k^{th}$ category, and $\sum_{k=1}^K \alpha_k$ indicates the total evidence for the prediction, and 
the belief and uncertainty mass represented by this Dirichlet distribution is:
%Given data $\{y_i, \bx_i\}_{i=1}^N$, the belief and uncertainty of a Dirichlet \gls{bba} is updated using the \textit{consensus operator} \citep{josang_consensus_2002}, and the resulting assignment corresponds exactly to the Dirichlet posterior distribution $P_{\balpha}(\bp)$ of a Bayesian Multinomial-Dirichlet model, which is computed using the Bayes' rule:
%\begin{align}
%    P_{\balpha}(\bp) &= 
%    \frac{P(y|\bp)P_{\balpha_0}(\bp)}{
%    \int P(y|\bp)P_{\balpha_0}(\bp) d\bp
%    }.
%    \label{eq:bayes}
%\end{align}
%where $P(y|\bp)$ is the Multinomial data likelihood (\ref{eq:multinom}), and $P_{\balpha_0}(\bp)$ is the Dirichlet prior distribution with prior parameters $\balpha_0 = [\alpha_{01}, \dots, \alpha_{0K}]$. Then the assignment of the updated Dirichlet \gls{bba} can be represented as \citep{josang_interpreting_2007}:
\begin{align}
    b_k = \frac{\alpha_k - 1}{\sum_{k=1}^K \alpha_k}, \quad u = \frac{K}{\sum_{k=1}^K \alpha_k}.
    \label{eq:opinion}
\end{align}
As shown, the uncertainty mass $\mu$ is inversely proportional to the total evidence and ranges between $[0, 1]$. If the model finds evidence for at least one category (i.e., $\alpha_k$ is large for any $k$), the uncertainty mass $\mu$ will be pulled toward zero, indicating confident prediction. On the other hand, if the model does not find evidence to support any of the known categories (i.e., $\alpha_k = 1$ for all $k$), the belief mass will all be zero and the uncertainty estimate is $\mu=K/K = 1$, i.e., a vacuous opinion.


==> section/section_old/idl_derivation.tex <==
Given data $\{y, \bx\}$ where $y$ follows a Multinomial distribution:
\begin{align*}
    P(y|\bp) \propto \prod_{k=1}^K p_k^{y_k} \qquad\mbox{where} \qquad \bp = [p_1, \dots, p_K],
\end{align*}
our goal is to infer the value of $\bp$ from data while properly quantifying our subjective uncertainty about the inference. 

The canonical method of incorporating uncertainty in to multivariate classification is through Bayesian update. That is, we assume a Multinomial model with Dirichlet prior:
\begin{alignat*}{3}
    \mbox{Model Likelihood:} \quad & y &&\sim P(y|\bp)  \propto \prod_{k=1}^K p_k^{y_k} \\
    \mbox{Prior Distribution:} \quad & \bp &&\sim P_0(\bp) \propto \prod_{k=1}^K p_k^{a_k - 1},
\end{alignat*}
where $P_0(\bp)$ is a Dirichlet distribution $Dir(\bp|\ba)$ with concentration parameters $\ba = [a_1, \dots, a_K]$. The posterior distribution of $P(\bp|y)$ is computed using the Bayes' rule:
\begin{align}
    P(\bp|y) &= \frac{P(y|\bp)P_0(\bp)}{\int_{\bp} P(y|\bp)P_0(\bp) d\bp}.
    \label{eq:bayes_rule}
\end{align}
To this end, the \textbf{\glsfirst{IDL}} computes this posterior distribution by leveraging the optimization view of Bayesian inference, that is, the posterior in (\ref{eq:bayes_rule}) is the solution to the below optimization problem \citep{zellner_optimal_1988, zhu_bayesian_2014, dai_provable_2016}:
\begin{align}
    P^*(\bp|y) &= \underset{Q \in \Dsc}{\mbox{argmin}} \; \Lsc(Q|\by) \qquad \mbox{where} \nonumber\\
    \Lsc(Q|\by) &:=  \Big[ -\int Q(\bp) * log P(y|\bp) d\bp \Big] + KL\Big( Q(\bp) || P_0(\bp) \Big).
    \label{eq:idl_bayes}
\end{align}
Here $\Dsc$ defines the space of \gls{PDF}s to optimize over. In this work, we define $\Dsc$ to be the space of the Dirichlet PDFs: 
$$\Dsc = \Big\{\frac{1}{B(\balpha)} \prod_{k=1}^K p_k^{\alpha_k-1} \Big| \balpha \in [1, \infty]^K \Big\},$$ 
since the posterior distribution of the Multinomial-Dirichlet model is known to be a Dirichlet distribution.

\vspace{1em}

We now derive the exact form of \gls{IDL} by computing the expression (\ref{eq:idl_bayes}) for the Multinomial-Dirichlet model.
\begin{itemize}
    \item First compute the likelihood term (i.e., the first squared bracket in (\ref{eq:idl_bayes})):
\begin{align*}
    -\int log P(y|\bp) * Q(\bp) d\bp 
    &= -\int \sum_{k=1}^K y_k \, log(p_k) * \frac{1}{B(\balpha)} \prod_{k=1} p_k^{\alpha_k-1}  d\bp\\
    &= - \int log(p_{k^*}) * \frac{1}{B(\balpha)} \prod_{k=1} p_k^{\alpha_k-1} d\bp \qquad \mbox{(where $k^*$ is the true category)}\\
    &= - \Big[\psi(\alpha_{k^*}) - \psi(\sum_{k=1}^K \alpha_k)\Big],
\end{align*}
where the last line follows due to the property of Dirichlet distribution: $E(log\, p_k) = \psi(\alpha_k) - \psi(\sum_k \alpha_k)$ \citep{minka_bayesian_2003}. Notice that this expression can be understood as the expectation of the cross entropy loss (i.e., the negative log likelihood of Multinomial distribution) with respect to a Dirichlet distribution, i.e., the Bayes risk \citep{murphy_machine_2012}. 

\item Now compute the prior term (i.e., the \gls{KL} term in (\ref{eq:idl_bayes})). 

Notice that this is essentially computing the \gls{KL} between two Dirichlet distributions $Q(\bp) = Dir(\bp|\balpha)$ and $P_0(\bp) = Dir(\bp|\ba)$:
\begin{align*}
    KL\Big( Q(\bp) || P_0(\bp) \Big) 
    &= \int \Big[ log Q(\bp) - log P_0(\bp) \Big] * Q(\bp) d\bp \\
    &= \int \Big[ log \frac{\prod_{k=1}^K p_k^{\alpha_k-1}}{B(\balpha)}  - log \frac{\prod_{k=1}^K p_k^{a_k-1}}{B(\ba)} \Big] * Q(\bp) d\bp\\
    &= -\Big[ log B(\balpha) - log B(\ba) \Big] + \int \sum_{k=1}^K (\alpha_k - a_k) log \, p_k * Q(\bp) d\bp\\
    &= -\Big[ log B(\balpha) - log B(\ba) \Big] + \sum_{k=1}^K (\alpha_k - a_k) E_Q(log \, p_k)\\
    &=  -\Big[ log B(\balpha) - log B(\ba) \Big] + \sum_{k=1}^K (\alpha_k - a_k) (\psi(\alpha_k) - \psi(\sum_k \alpha_k))
\end{align*}
where we again used the property $E(log\, p_k) = \psi(\alpha_k) - \psi(\sum_k \alpha_k)$. With a bit abuse of notation, we will write this term as $KL(\balpha || \ba)$.
\end{itemize}
Finally, by combining both terms, we have reached the expression for the \glsfirst{IDL} loss:
\begin{align*}
    \Lsc(\balpha|\by) &= - \Big[\psi(\alpha_{k^*}) - \psi(\sum_{k=1}^K \alpha_k)\Big] + KL(\balpha || \ba)
\end{align*}

==> section/section_old/injective.tex <==
\begin{proposition}[Lipschitz residual network is distance preserving]
\end{proposition}

Application: Issue with Model Architecture?

\begin{enumerate}
    \item Out-of-domain. Confidence associated with distance to data support. This distance needs to be reflected properly in the hidden space.
    \item Calibration \citep{gneiting_probabilistic_2014}. 
    Intuitively: Needs to properly represent the underlying data generation mechanism across feature space, otherwise over-confidence on wrong predictions (e.g., confidently wrong case where model systematically predict 0 for 9 because it observed a "circle pattern" and ignore the rest of the information from the input, which leads to mis-calibration).
    Requires distributional match through proper distributional transform. Otherwise destroys information.
    Formally, need to properly represent probability integral transform for the input space, which needs the function to be invertible. 
\end{enumerate}

Connection between Lipschitz Condition and Uncertainty Performance:
\begin{enumerate}
    \item Uncertainty concentration \citep{ciosek_conservative_2020}
    \item Distance Preservation - Injectivity \citep{behrmann_invertible_2019, behrmann_invertibility_2019}
\end{enumerate}

Approaches to ensure Lipschitz condition:
\begin{enumerate}
    \item Invertible Network \citep{jacobsen_i-revnet_2018}, difficult to train (memory) \cite{van_amersfoort_simple_2020}, performance \citep{ardizzone_exact_2020}, invertibility not guaranteed \citep{behrmann_invertibility_2019}
    \item Gradient Penalty \cite{van_amersfoort_simple_2020}
    \item Spectral Normalization \citep{miyato_spectral_2018, behrmann_invertibility_2019}.
\end{enumerate}


==> section/section_old/intro_v0.tex <==
Scalable and high-quality methods for quantifying model uncertainty is crucial for deploying \gls{DNN}-based systems in industrial-scale,  real-world applications. The examples range from object recognition in autonomous driving \citep{feng_towards_2018}, to intent understanding in conversational system \citep{zheng_out--domain_2019}, to real-time ad click prediction in computational advertising \citep{van_aken_challenges_2018}. For these applications, a  machine-learning services' latency, accuracy and reliability are all of paramount importance. As a result, an ideal \gls{UQ} method should not only reliably capture different types of uncertainties in a \gls{DNN} model, but also achieve comparable predictive accuracy and inference speed with that of a deterministic \gls{DNN}.

A variety of methods have been proposed for quantifying deep learning uncertainty. 
%These methods usually proceed by imposing certain \textit{a priori} probabilistic structure for a \gls{DNN} model $y=f(\bx)$, and quantify uncertainty by computing the \textit{a posteriori} predictive distribution $P(y|f(\bx))$ from data. The specific methods differ in their choices of the probabilistic structure: 
The most common class of approaches 
%imposes explicit priors on the neural network, i.e., by formulating a \gls{BNN}, and then 
focuses on computing the posterior distribution of a \gls{BNN}  \citep{blundell_weight_2015, louizos_structured_2016, wu_deterministic_2018, sun_functional_2019}. A second and more recent class of approaches re-purposes deterministic training techniques (e.g., dropout \citep{gal_dropout_2016}, stochastic averaging \citep{maddox_simple_2019}, random initiation \citep{lakshminarayanan_simple_2017, wilson_bayesian_2020}) as implicit Bayesian inference, and generates predictive distribution by ensembling multiple stochastic realizations of deterministically-trained \gls{DNN}s. 
%The notable examples in this class include \gls{MCD}\citep{gal_dropout_2016}, \gls{SWAG} \citep{maddox_simple_2019} and Deep Ensemble \citep{lakshminarayanan_simple_2017, wilson_bayesian_2020}. %\footnote{Although commonly known as a non-Bayesian technique, Deep Ensemble has recently been shown to be an implementation of \gls{BMA}\citep{wilson_bayesian_2020} .}. 
%We present these methods under an unified Bayesian view in Section \ref{sec:methods_review}.
However, despite the steady progress made by these methods on various uncertainty benchmarks, they often fall short in either predictive accuracy or inference latency when compared to a deterministic \gls{DNN}, due to the \gls{BNN} model's sensitivity to prior misspecification, or the Monte-Carlo nature of the ensemble algorithm \citep{snoek_can_2019, wenzel_how_2020}. 
% For example, \gls{BNN} with explicit priors were shown to yield  systematically worse predictions compared to a determinstic neural network even under exact MCMC inference \citep{wenzel_how_2020}. The ensemble approaches require $K$ forward passes to compute predictive distribution, effectively increasing inference latency by a multiplicative factor $K$, rendering them impractical for large-scale, real-time applications.

To this end, a third class of approaches, which we term the single-model method, has emerged as an attractive alternative \citep{malinin_predictive_2018, sensoy_evidential_2018}. Building on the \gls{EB} principle, these methods compute the predictive distribution as the closed-form posterior of a Multinomial-Dirichlet model conditional on the logits, 
%perform exact posterior inference for the parameters of the last layer, 
and learn the earlier-layer parameters through \gls{MAP} training \citep{efron_bayes_2019}. As a result, the Bayesian inference is trivialized into scalable \gls{SGD} training with respect to a loss function induced by the Bayesian posterior \citep{dai_provable_2016}. The resulting model are shown to deliver similar predictive performance and inference latency to that of a deterministic \gls{DNN} \citep{malinin_reverse_2019}, yield meaningful estimates of data and model uncertainty \cite{malinin_predictive_2018}, and promising performance for uncertainty tasks in machine vision \citep{sensoy_evidential_2018}. 

However, the current single-model approaches to \gls{UQ} are unsatisfying in three aspects. On the methodology side, the single-model approaches suffer a fundamental limitation of lacking model diversity. This is because the model's uncertainty estimate is derived from a single \gls{MAP}-trained network, therefore  under-representing the inherent weight stochasticity that arise during the training process, which is part of the model uncertainty \citep{blundell_weight_2015, malinin_ensemble_2020}. As a result, the single-model methods often resort to additional adversarial training on \gls{OOD} data to attain robust performance, incurring undesirable technical debt for a industrial system \citep{lee_training_2018, malinin_predictive_2018, malinin_prior_2018, malinin_reverse_2019}. On the theoretical side, the frequentest properties of the loss function induced by the Bayesian posterior is not well-understood.  How these Bayesian-induced loss function compare against its frequentest counterparts (i.e., the \gls{CE} loss), and how such difference impacts the model behavior is an important problem both in theory and in practice. Finally, on the practical side, the work on single-model methods so far have been tested mainly on classic machine vision architecture (e.g, LeNet, VGG-16). Given their promise for real-world applications, it is important to gain a thorough understanding of the method's empirical performance on practical modern networks (e.g., ResNet and Transformer), across data modalities beyond machine vision, and on metrics for both data and model uncertainty.


In this work, we explore the limit of scalable uncertainty quantification for \gls{DNN} by understanding how far can we push the single-model approach to achieve all three criteria of an ideal \gls{UQ} method: accurate prediction, fast inference speed, and high-quality uncertainty quantification. Our goal is to arrive at a reliable \gls{UQ} approach amendable for industrial-scale application with well-understood properties. To achieve this, we present methodology innovation to address the single-model approach's limitation in lacking intrinsic diversity, and conduct both theoretical and empirical investigations to understand its performance in prediction and in \gls{UQ}.
Specifically, we make three contributions: 

    $\bullet$ \textbf{Methodology}: We propose a \gls{GP}-based re-formulation of the single-model approach, addressing its fundamental limitation in lacking diversity. This re-formulation is based on a novel construction of \gls{GP} as a neural network layer, which is derived using the random-feature expansion of the model's Laplace posterior \citep{rahimi_random_2008, rasmussen_gaussian_2006, riihimaki_laplace_2014}. This novel \gls{GP} construction allows the model to be trained end-to-end using minibatch \gls{SGD} and comes with an approximation guarantee to the exact posterior  \citep{avron_random_2017, choromanski_geometry_2018,  kass_validity_1990}. As a result, the \gls{DNN} is turned into a deep Dirichlet-\gls{GP} model whose posterior estimate encodes proper stochastic diversity and yet can be computed in closed-form. 

    $\bullet$ \textbf{Theory}: We analyze the single-model method's behavior both in prediction and in \gls{UQ}. Specifically, we conduct a frequentest analysis of the Bayesian-induced loss function under the single-model method, revealing its connection with the standard deterministic objective (i.e., the \gls{CE} loss). We also conduct a decomposition of the model's overall uncertainty into data and model uncertainty, making it explicit the contribution of different model components to the model's overall \gls{UQ} ability.
    
    $\bullet$ \textbf{Practice}: We conduct a thorough empirical investigation of the single-model method's performance,  benchmarking it against \gls{BNN} and ensemble approaches across multiple data modalities (vision, language and categorical), on practical architecture (e.g., ResNet and Transformer), and with respect to quality metrics for both data and model uncertainty. We show that, {\color{red} XXX}.

Also check \citep{ciosek_conservative_2020}.

\begin{itemize}
    \item Need of Deep Learning Uncertainty.
    \item State-of-the-art approaches: Bayesian and Deep Ensemble.
    \begin{itemize}
        \item \citep{zellner_optimal_1988}.
        \item Caveat in real-time, large-scale applications. (training cost, inference latency, technical debt).
    \end{itemize}
    \item Motivates single model approaches.
    \begin{enumerate}
        \item before venturing into the thicket of developing another single-model method:
        \begin{itemize}
            \item Bayesian inference on last layer \citep{snoek_scalable_2015}\citep{riquelme_deep_2018}
            \item Orthogonal Certificates
            \citep{tagasovska_single-model_2019}
            \item Prior Networks \citep{malinin_predictive_2018}, Evidential Learning \citep{sensoy_evidential_2018}.
        \end{itemize}
        \item would like to first understand the theoretical \textbf{Possibility} of this avenue. Is it possible for a single model to be competitive with Bayesian / ensemble in uncertainty quantification?
        \item To understand this, we need to answer:
        \begin{enumerate}
            \item how to understand the problem of uncertainty estimation rigorously from a learning theory perspective?
            \item what is the characterization of an optimal solution to the uncertainty estimation?
            \item can such characterization be achieved using a single model?
        \end{enumerate}
    \end{enumerate}
    \item The first goal of this work is an attempt to answer the above questions. In Section \ref{sec:theory}, we 
    \begin{enumerate}
        \item 
        \item mathematical tools are classic. Insights and implications for uncertainty quantification in deep learning, we believe, is new.
    \end{enumerate}
    \item The second goal of this work is to validate the theoretic results in Section \ref{sec:theory} by proposing \gls{SNGP}, a simple method that improves the distance-awareness ability of modern DNNs.
\end{itemize}

\begin{itemize}
    \item What is lacking:
    \item A principled understanding of the explicit connection between the property of a proposed deterministic \gls{DNN} and the final objective in uncertainty quantification, e.g., the Brier score or the calibration error.
\end{itemize}
    
\jzl{write down the flow here and link to Sections}

In this work, we would like to take a principled approach to the uncertainty estimation problem.


To this end, the goal of this paper is to improve the both the theory and the practice of single-model methods for high-quality uncertainty quantification. Specifically, 
\begin{itemize}
\item We identify distance awareness as a necessary theoretical property for a deterministic DNN to achieve (minimax) optimal performance in uncertainty quantification.
\item We propose \gls{SNGP}, a simple augmentation method for deep neural networks to improve their ability in distance awareness. In practice, \gls{SNGP} involves only adding a regularizer to the weight matrix and replacing the activation function of the penultimate layer. As a result, it improves uncertainty quantification ability of DNN while preserving its predictive accuracy and inference latency. 
\item We interrogate the \gls{SNGP}'s performance in uncertainty quantification on non-trivial modern architectures (ResNet and BERT) and across data modalities. We show that, despite being a single-model method, \gls{SNGP} can be competitive or slightly outperform Deep Ensemble. 
\end{itemize}



==> section/section_old/intro_v1.tex <==
Efficient methods that reliably quantifies a \gls{DNN}'s predictive uncertainty are important for deep-learning-based systems in industrial-scale, real-world applications. The examples include object recognition in autonomous driving \citep{feng_towards_2018}, real-time intent understanding in conversational system \citep{zheng_out--domain_2020}, and online ad click prediction in computational advertising \citep{van_aken_challenges_2018}. For these applications, the system's accuracy, reliability and latency are all of paramount importance.

The current state-of-the-art methods for \gls{UQ} for deep learning include \gls{BNN} \citep{neal_bayesian_1996}, \gls{MCD} \citep{gal_bayesian_2015} and deep ensembles \citep{lakshminarayanan_simple_2017}. These approaches adopt a principled interpretation as performing probabilistic inference with an explicit or implicit prior 
\citep{gal_bayesian_2015, wilson_bayesian_2020}, and empirically lead to concrete improvements in calibration and \gls{OOD} robustness when compared to a deterministic baseline
\citep{ovadia_can_2019}.
However, a common caveat of these approaches is their high training and inference cost, mainly due to the need of using Monte Carlo sampling or ensemble averaging. This shortcoming has limited their practicality in industrial-scale applications, and motivated researchers to study methods that use only a single deterministic model \citep{malinin_predictive_2018, sensoy_evidential_2018, tagasovska_single-model_2019}.
The ambition is to maintain the accuracy and latency of a deterministic \gls{DNN}, and yet achieve uncertainty performance (e.g., calibration and \gls{OOD} detection) that is competitive with that of a deep ensemble. 
%There exists a few works on this direction, with the examples include orthogonal certificates \citep{tagasovska_single-model_2019}, prior networks \citep{malinin_predictive_2018} and evidential deep learning \citep{sensoy_evidential_2018}. 
However, what is not yet clear is the \textbf{theoretical admissibility} of this avenue, i.e., is it even theoretically possible for a single model to attain an uncertainty performance that is comparable to, say, a Deep Ensemble? 
%Furthermore, assuming it is attainable, what are the necessary properties of a deterministic \gls{DNN} that is needed to achieve optimal performance?
%Before venturing into the thicket of developing another single-model method, in this work, we would like to take a different approach by first understanding the \textbf{theoretical possibility} of this avenue, i.e., is it even possible for a single model to attain a theoretically optimal performance in uncertainty quantification? 
\imp{\textbf{Deepak}:Since people have already pointed out that intro is perhaps too verbose, I would suggest this entire para can be removed, and/or merged with the next one.} 
To address this question with sufficient rigor, there are a sequence of questions that we need to answer: \textbf{(a)} How to understand the problem of uncertainty estimation from a learning theory perspective? \textbf{(b)} What is the characterization of an optimal solution to this uncertainty estimation problem? \textbf{(c)} Can such characterization be achieved using a single deep learning model?

This work answers the aforementioned questions by making contributions along the below three goals: theoretical, methodological and experimental.
\textbf{(a)} We first formulate the single-model uncertainty estimation problem as a minimax learning problem with respect to a suitable uncertainty loss, and derive its optimal solution in closed form. We then establish \textit{input distance awareness} %\imp{Shreyas:could we use a shorter moniker/abbreviation for input distance-awareness? It's repeated a lot throughout the text and could help the flow to have an abbreviation} 
as an important property for a model to achieve high-quality uncertainty estimation. \textbf{(b)} Next, we propose a simple modification to a \gls{DNN}, which we name \textit{\glsfirst{SNGP}}, to improve its ability to preserve the \textit{input distance awareness}.  
\textbf{(c)} Finally, we experimentally demonstrate that such characterization can be achieved by a single model on a suite of  vision and language understanding tasks with non-trivial modern architectures (ResNet and BERT). 
We show that the \gls{SNGP} approach attains an uncertainty performance (e.g., calibration and \gls{OOD} detection) that is competitive with that of a deep ensemble, while maintaining the accuracy and latency of a single deterministic \gls{DNN}. while maintaining the accuracy and latency of a single deterministic \gls{DNN}.\imp{\textbf{Deepak}:last sentence is a possible repeat}

%\tbw{Consider shortening the next three paragraphs since you're going into quite a bit of detail later.  For example: This work makes contributions along the three goals: theoretical, methodological, and experimental. We first formulate the single-model uncertainty estimation problem as a minimax learning problem with respect to a suitable uncertainty loss and then  derive its optimal solution in closed form, and establish \textit{input distance awareness} as an important property for a model to achieve high-quality uncertainty estimation.  Next, we propose small modifications to a DNN, which we name \textit{\gls{SNGP}}, to improve its ability to preserve \textit{input distance awareness}.  Finally, we demonstrate that such characterization can be achieved by a single model on a suite of 2-dimensional classification benchmarks, while maintaining the accuracy and latency of a single deterministic \gls{DNN}.}

%Consequently, the \textbf{first goal} of this work is theoretical: to achieve a principled understanding of the single-model uncertainty estimation problem by answering the aforementioned questions (Section \ref{sec:theory}). Specifically, we first  \textbf{(a)} formalize the problem of uncertainty estimation as a minimax learning problem with respect to a suitable uncertainty loss (i.e., the Brier risk) (Equation \ref{eq:minimax_loss}), and then  derive its optimal solution in closed form, hence verifying that the uncertainty learning problem is well-posed and comes with a simple solution that is a practically attainable  (Proposition \ref{thm:minimax}). By doing so, we \textbf{(b)} identify \textit{input distance awareness} (i.e., the model’s ability in quantifying the distance of a testing example from the training data \textit{in the input space}) as an important property for a model to achieve high-quality (minimax optimal) uncertainty estimation.  Finally, for a deep learning model, we \textbf{(c)} propose two simple conditions for it to achieve \textit{input distance awareness}. That is, for a neural network $logit(\bx) = g \circ h(\bx)$, its output layer $g$ should be \textit{distance-aware}, and its embedding function $h$ should be \textit{distance-preserving}, i.e., bi-Lipschitz (Definition \ref{def:dp}).

%Based on the derived theoretical insight, the \textbf{second goal} of this work is methodological: in Section \ref{sec:method}, we propose  \textit{\gls{SNGP}}, a simple method that improves a \gls{DNN}'s ability in \textit{input distance awareness} (Section \ref{sec:method}). Specifically, \gls{SNGP} makes the output layer $g$ \textit{distance-aware} by replacing the dense layer with a \gls{GP} layer, and introduces a novel Laplace-based \gls{RFF} approximation scheme to make the \gls{GP} training linearly scalable (Section \ref{sec:gp}). \gls{SNGP} then makes the embedding function $h$ \textit{distance preserving} by applying spectral normalization to the neural network weights, which effectively ensures the distance preservation property by making the embedding function bi-Lipschitz (Proposition \ref{thm:resnet_lipschitz}) (Section \ref{sec:sn}). As a result, \gls{SNGP} turns a \gls{DNN} into a \glsfirst{GP} model with distance-preserving feature map, bringing concrete benefit to uncertainty estimation, yet adding only negligible computational overhead to the training and inference pipeline of a standard \gls{DNN}. 

%\tbw{To demonstrate that such characterization can be achieved with a single deep model, we study how \gls{SNGP}'s uncertainty estimate... } We study both qualitatively and quantitatively the property \gls{SNGP}'s uncertainty estimate on a suite of 2-dimensional classification benchmarks (Section \ref{sec:exp_2d}, Figure \ref{fig:2d_exp}) and on vision and language understanding tasks with non-trivial modern architectures (ResNet and BERT) (Section \ref{sec:exp_ml}). Experimental evidence suggests that the \textit{input distance awareness} property brings concrete benefit to a model's ability in uncertainty quantification. By encouraging such property, the \gls{SNGP} approach attains a uncertainty performance (e.g., calibration and \gls{OOD} detection) that is competitive with that of a deep ensemble, while maintaining the accuracy and latency of a single deterministic \gls{DNN}.

==> section/section_old/main_old.tex <==




\paragraph{measure}

\paragraph{design specs}
parameter distribution $p(\btheta | \Dsc)$

\begin{enumerate}
    \item domain-aware formulation
    \item OOD detection: distance-awareness.
    \item Calibration: temperature scaling. 
\end{enumerate}

\begin{lemma}[Distance Awareness]
\end{lemma}

\section{Distance Awareness is Necessary for Uncertainty Quantification}


\begin{lemma}[Calibration Error]
\end{lemma}

\begin{itemize}
    \item Accurate Distribution Learning implies Calibration
    \item IND/OOD decomposition.
\end{itemize}

\begin{proposition}[Minimax Predictive Distribution for Calibration Error]
\end{proposition}


\section{Method}

Two conditions.

\subsection{\gls{NGP} Layer: Scalable Layer for Distance Awareness}

\gls{NGP} Layer: simple neural network module with clear arithmetic semantics to satisfy both of the above design requirements: Distance awareness / Adaptive scaling.

Specifically, 
\begin{enumerate}
    \item Train Gaussian process with shift-invariance kernel to incorporate distance awareness.
    \item At inference time, scaling prediction with posterior variance. (dampen the magnitude of the in-confident prediction when lack data support)
    \item Formulate a simple network module that can be trained end-to-end with minimal change to the existing system, and minimal change to the predictive accuracy and inference speed. Random feature expansion of Laplace posterior.
\end{enumerate}


\paragraph{Normalized Gaussian Process}

\paragraph{Closed-form Posterior Inference via Laplace Approximation}

\paragraph{Summary}

\begin{enumerate}
    \item Behavior of \gls{NGP} Uncertainty.
    \item Interpretation as a Manifold \gls{GP} \citep{calandra_manifold_2014} . 
\end{enumerate}

\clearpage

\subsection{Distance-preserving Neural Mapping via Lipschitz Condition}
\label{sec:injective}

\input{"./section/injective"}



\newpage
\section{\gls{NGP} Layer v.s. Other Single-Model Methods}
\label{sec:related}
\input{"./section/related"}




\clearpage
\section{Experiments}

==> section/section_old/nips_style.tex <==
\section{Submission of papers to NeurIPS 2020}

NeurIPS requires electronic submissions.  The electronic submission site is
\begin{center}
  \url{https://cmt3.research.microsoft.com/NeurIPS2020/}
\end{center}

Please read the instructions below carefully and follow them faithfully.

\subsection{Style}

Papers to be submitted to NeurIPS 2020 must be prepared according to the
instructions presented here. Papers may only be up to eight pages long,
including figures. Additional pages \emph{containing only a section on the broader impact, acknowledgments and/or cited references} are allowed. Papers that exceed eight pages of content will not be reviewed, or in any other way considered for
presentation at the conference.

The margins in 2020 are the same as those in 2007, which allow for $\sim$$15\%$
more words in the paper compared to earlier years.

Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.

\subsection{Retrieval of style files}

The style files for NeurIPS and other conference information are available on
the World Wide Web at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2020.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.

The only supported style file for NeurIPS 2020 is \verb+neurips_2020.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}

The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.

\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS.

At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.

The file \verb+neurips_2020.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.

The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.

The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.

For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.

Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

All headings should be lower case (except for first word and proper nouns),
flush left, and bold.

First-level headings should be in 12-point type.

\subsection{Headings: second level}

Second-level headings should be in 10-point type.

\subsubsection{Headings: third level}

Third-level headings should be in 10-point type.

\paragraph{Paragraphs}

There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone.

\subsection{Citations within the text}

The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.

The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}

If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2020+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}

If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2020}
\end{verbatim}

As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous.''

\subsection{Footnotes}

Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).

Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}

\subsection{Figures}

\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}

All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.

You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.

\subsection{Tables}

All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.

Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.

Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\section{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PDF files}

Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''

Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.

\begin{itemize}

\item You should directly generate PDF files using \verb+pdflatex+.

\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.

\item The IEEE has recommendations for generating PDF files whose fonts are also
  acceptable for NeurIPS. Please see
  \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}

\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.

\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.

\end{itemize}

If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.

\subsection{Margins in \LaTeX{}}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})

A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.


\section*{Broader Impact}

Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
biases in the data. If authors believe this is not applicable to them, authors can simply state this.

Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}

\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare 
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work). 
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2020/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}

\section*{References}

References follow the acknowledgments. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
{\bf Note that the Reference section does not count towards the eight pages of content that are allowed.}
\medskip

\small

[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.

[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.

[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.


==> section/section_old/old.tex <==




\paragraph{measure}

\paragraph{design specs}
parameter distribution $p(\btheta | \Dsc)$

\begin{enumerate}
    \item domain-aware formulation
    \item OOD detection: distance-awareness.
    \item Calibration: temperature scaling. 
\end{enumerate}

\begin{lemma}[Distance Awareness]
\end{lemma}

\section{Distance Awareness is Necessary for Uncertainty Quantification}


\begin{lemma}[Calibration Error]
\end{lemma}

\begin{itemize}
    \item Accurate Distribution Learning implies Calibration
    \item IND/OOD decomposition.
\end{itemize}

\begin{proposition}[Minimax Predictive Distribution for Calibration Error]
\end{proposition}

\paragraph{Notation and Problem Setup}
\begin{itemize}
    \item Learning setting: 
    \begin{itemize}
        \item Data generation distribution $p^*(y|x)$ for $x \in \Xsc$. Training data is collected from a training domain $X_{\texttt{train}} \in \Xsc$.
        \item During training, the model only observes an empirical version of in-domain distribution $p^*(y|x, x \in X_{\texttt{train}})$.
        \item However, during testing, the model is asked to construct a predictive distribution $p(y|x)$ for the entire input space $x \in X$. 
        So that it minimizes some metric of interest.
    \end{itemize}
    \item In the context of uncertainty quantification, a suitable metric is Brier Score
    \begin{itemize}
        \item Comprehensively captures both sharpness and calibration.\citep{degroot_comparison_1983}
        \item Upper bounds the calibration error.
    \end{itemize}
\end{itemize}
    
\paragraph{Uncertainty estimation via Game-theoretic Lens}
    \begin{itemize}
        \item Since the true distribution is unknown, a principled strategy is to construct predictive distribution such that it minimizes the worst-case Brier Score.
        \item It is natural to study this problem from a game-theoretic perspective. Specifically, we cast uncertainty quantification as a prediction game against Nature, where the nature's true strategy $p^*(y|x)$ is only partially known, and the goal of the game is to identify a minimax strategy $p(y|x)$ that minimizes the worst-case uncertainty loss (i.e., the Brier Score), i.e., we'd like to find $p(y|x)$ such that:
        $$\hat{p} = \underset{p \in \Psc}{\operatorname{arginf}}  \Big[ \sup_{p^* \in \Psc^*} \; S(p^*, p) \Big] $$
    \item Interestingly, by a simple application of the maximum entropy principle.  Minimax Optimal Predictive Distribution for Brier Score by Maximum Entropy Principle (Proposition 1)
    \begin{itemize}
        \item A generalization of classic maximum entropy principle for Brier score \citep{grunwald_game_2004}. Application to the context of uncertainty quantification for deep learning is new.
        \item Theoretical ideal, but offer principled design guideline: sharpness when in-domain, and maximum entropy when out-of-domain. i.e., the principle of insufficient reason \citep{murphy_machine_2012, jaynes_probability_2003}. Hinted in previous work \citep{malinin_prior_2018} but not formalized.
        \item practical example: Gaussian Process with shift-invariant kernel, posterior uncertainty reflects distance from the training data, revert to prior \citep{rasmussen_gaussian_2004, liu_accurate_2019}. True for both regression and classification cases.
    \end{itemize}
    \end{itemize}
    
\paragraph{Distance Awareness as a Necessary Condition. (Definition 1)}
\begin{itemize}
    \item To this end, the interest of this work is to study.
    
    To this end, our interest is to understand what mathematical properties of the neural network $p(\bx)= g \circ h(\bx)$ are necessary for it to achieve high-quality uncertainty quantification. In this work, we consider the so-called \textit{distance awareness} property:

    \item Definition of Distance Awareness.
    
\begin{definition}[Distance Awareness]
$ $\\
Consider a predictive distribution $p(y|\bx)$ trained on a domain $\Xsc_{\textup{\texttt{train}}} \subset \Xsc$, where $(\Xsc, ||.||_X)$ is the input data manifold equipped with a suitable distance measure $||.||_X$. We say $p(y|\bx)$ is \underline{distance aware} if it can output an uncertainty function $u(\bx)$, such that:
$$u(\bx) = f_{\mbox{\tiny \textup{\texttt{monotonic}}}}\big(
d(\bx, \Xsc_{\textup{\texttt{train}}})\big)$$
where $f_{\mbox{\tiny \textup{\texttt{monotonic}}}}$ is a monotonic function and $d(\bx, \Xsc_{\textup{\texttt{train}}})$ is the distance between a testing example $\bx$ from the training data domain, i.e., $d(\bx, \Xsc_{\textup{\texttt{train}}}) = inf_{\bx' \in \Xsc_{\textup{\texttt{train}}}} ||\bx - \bx'||_X$. 
\end{definition}

    \item Next question. How to construct $p$ to achieve distance awareness? Look deeper into structure of a neural network. Decomposition into embedding function $h$ and output layer $g$.
    
    Modern neural networks $p(\bx) = g \circ h(\bx)$ are commonly composed of a embedding function $h$ and a output layer $g$, such that the embedding function $h: \Xsc \rightarrow \Hsc$ maps $\bx$ from input space $\Xsc$ to a hidden representation space $\Hsc$, and the output layer $g: \Hsc \rightarrow \Ysc$ maps the hidden-space representation $h(\bx)$ to the output space. For example, in a ResNet50, the embedding function $h(.)$ is the stack of residual blocks and pooling layers, and $g(.)$ is the final 1000-dimensional dense layer with softmax activation function \citep{he_deep_2016}.
    
    \item Condition on $h$ (distance preservation) and $g$ (distance aware).
    
\begin{definition}[Distance Preservation]
$ $\\
For $h:\Xsc \rightarrow \Hsc$ defined on metric spaces $(\Xsc, ||.||_X)$ and $(\Hsc, ||.||_H)$, we say the embedding function $h$ is \underline{distance preserving} if there exists $0 < L_1 < L_2$, such that for any $\bx_1, \bx_2 \in \Xsc$:
$$ L_1 * ||\bx_1 - \bx_2||_X \leq ||h(\bx_1) - h(\bx_2)||_H \leq L_2 * ||\bx_1 - \bx_2||_X,$$
i.e., the projection $h$ preserves the distance between the data points.
\end{definition}

    
    \item Not guaranteed in general (adversarial examples \citep{jacobsen_excessive_2018}, unscaled inner product distance to decision boundary Figure \ref{fig:2d_exp_oval_deepens} and \ref{fig:2d_exp_moon_deepens}). Motivates the Method Section.
\end{itemize}

\subsection{Distance-aware Predictive Distribution achieves Optimal Calibration Error}

Since the data $\bx_{\texttt{test}}$ can be sampled anywhere from the entire input space $\Xsc$, the model needs to construct a full predictive distribution for the entire input space, such that, 
\begin{alignat}{6}
    p(y |\bx) 
    &= p(y|\bx, \bx \in \Xsc_{\texttt{train}})&& * p(\bx \in \Xsc_{\texttt{train}}) 
    && + p(y|\bx, \bx \not\in \Xsc_{\texttt{train}})&& * p(\bx \not\in \Xsc_{\texttt{train}})
    \nonumber\\
    &= 
    \quad p_{\texttt{IND}}(y|\bx)&& * p(\bx \in \Xsc_{\texttt{train}}) 
    && + 
    \quad p_{\texttt{OOD}}(y|\bx)&& * p(\bx \not\in \Xsc_{\texttt{train}}).
\end{alignat}

To assesses a model's reliability in this open-world scenario, a standard measure is the \textit{calibration error} (CE) \citep{degroot_comparison_1983, gneiting_probabilistic_2007, murphy_reliability_1977, kumar_verified_2019}. Given all the cases $\bx \in \Xsc$ where the model outputs predictive probability $\hat{p}(\bx)=max_k \, p(y_k|\bx)=p$, CE compares the difference between a model's predictive probability score $p$ and its actual probability of being correct:
\begin{definition}[Calibration Error]
\begin{align}
CE[p(y|\bx)] = \sqrt{\mathbb{E}\Big[ 
    \Big( \mathbb{P} \big( y^*=\hat{y} | \hat{p}(\bx) = p \big) - p \Big)^2
\Big]}.    
\end{align}
\end{definition}
If $CE[p(y|\bx)]=0$, then the model $p(y|\bx)$'s predictive score $p$ has a direct correspondence with its actual predictive accuracy, indicating a trustworthy prediction.

\begin{proposition}[$p(y|\bx)$ Minimizes Worst-case Calibration Error]
\end{proposition}

\section{Method}

Two conditions.

\subsection{\gls{NGP} Layer: Scalable Layer for Distance Awareness}

\gls{NGP} Layer: simple neural network module with clear arithmetic semantics to satisfy both of the above design requirements: Distance awareness / Adaptive scaling.

Specifically, 
\begin{enumerate}
    \item Train Gaussian process with shift-invariance kernel to incorporate distance awareness.
    \item At inference time, scaling prediction with posterior variance. (dampen the magnitude of the in-confident prediction when lack data support)
    \item Formulate a simple network module that can be trained end-to-end with minimal change to the existing system, and minimal change to the predictive accuracy and inference speed. Random feature expansion of Laplace posterior.
\end{enumerate}


\paragraph{Normalized Gaussian Process}

\paragraph{Closed-form Posterior Inference via Laplace Approximation}

\paragraph{Summary}

\begin{enumerate}
    \item Behavior of \gls{NGP} Uncertainty.
    \item Interpretation as a Manifold \gls{GP} \citep{calandra_manifold_2014} . 
\end{enumerate}

\clearpage

\subsection{Distance-preserving Neural Mapping via Lipschitz Condition}
\label{sec:injective}

\input{"./section/injective"}



\newpage
\section{\gls{NGP} Layer v.s. Other Single-Model Methods}
\label{sec:related}
\input{"./section/related"}




\clearpage
\section{Experiments}

==> section/section_old/related_old.tex <==
\subsection{\gls{GP}-\gls{DNN} and Invertible Network for Uncertainty Quantification}

\gls{GP}-\gls{DNN}
\begin{enumerate}
    \item Uncertainty: Calibration: \citep{tran_calibrating_2019} using  \gls{MCD}.
    \item \gls{OOD}/Novelty Detection: \citep{domingues_deep_2018}
    \item Adversarial Robustness / Domain Transfer: \citep{bradshaw_adversarial_2017}
\end{enumerate}
No uncertainty decomposition, not highlighting the importance of model architecture in deep network.

Invertibility
\begin{enumerate}
    \item Calibration and \gls{OOD}: \citep{ardizzone_exact_2020}, \citep{nalisnick_hybrid_2019}
    \item Adversarial Robustness:  \citep{jacobsen_excessive_2018}
\end{enumerate}

\subsection{Scalable \gls{GP} Methods}
Combination of Laplace approximation and Random Fourier Feature for a non-standard likelihood (integrated log posterior of a Multinomial-Dirichlet model). Formulated as a neural network module amendable to mini-batch update.

\begin{enumerate}
    \item Laplace approximation for multinomial likelihood:
\citep{williams_bayesian_1995}
\citep{rasmussen_gaussian_2006}
\citep{riihimaki_gaussian_2010}
Despite theoretically worse approximation quality for the full posterior \citep{nickisch_approximations_2008}. Strong candidate for neural formulation, tight connection with frequentest training and good computational efficiency.
    \item Random Fourier Feature in deep learning 
    \begin{enumerate}
        \item Frequentest: 
        model \citep{mehrkanoon_deep_2018}
        Theory
        \citep{kawaguchi_deep_2018}. better generalization.
        \item Bayesian (GP). 
        \begin{enumerate}
            \item Prediction: Mostly use \gls{VI} and focus on prediction, e.g.,  Mean-field \gls{VI} \citep{cutajar_random_2017} \citep{hensman_scalable_2015}
    Structured \gls{VI} \citep{hensman_variational_2018}, goals are mostly prediction. inferior approximation for posterior variance. challenge in computation due to complicated optimization landscape.
            \item Uncertainty: Calibration: \citep{tran_calibrating_2019} using  \gls{MCD}.
            \item \gls{OOD}: \citep{domingues_deep_2018}
        \end{enumerate}
    \end{enumerate}

\end{enumerate}

Different Model Formulation
\begin{enumerate}
\item Gamma augmentation: \citep{milios_dirichlet-based_2018}
\item Polya-gamma augmentation: \citep{linderman_dependent_2015}
\end{enumerate}


\section{\textbf{Even older version}}

GP-DNN Mixture 
\begin{enumerate}
    \item DKL \citep{wilson_stochastic_2016}
    \item GP-DNN \citep{bradshaw_adversarial_2017} \citep{hensman_scalable_2015}
    \item CNN-RFF-MCD \citep{tran_calibrating_2019}
    \item DUQ \citep{van_amersfoort_simple_2020}
\end{enumerate}

\gls{ID} loss:
\begin{enumerate}
    \item Prior Networks \citep{malinin_predictive_2018}
    \item Evidential Learning \citep{sensoy_evidential_2018}
\end{enumerate}


\subsection{Related Work}
\subsubsection{\gls{GP}-\gls{DNN} and Invertible Network for Uncertainty Quantification}

\gls{GP}-\gls{DNN}
\begin{enumerate}
    \item Uncertainty: Calibration: \citep{tran_calibrating_2019} using  \gls{MCD}.
    \item \gls{OOD}/Novelty Detection: \citep{domingues_deep_2018}
    \item Adversarial Robustness / Domain Transfer: \citep{bradshaw_adversarial_2017}
\end{enumerate}
No uncertainty decomposition, not highlighting the importance of model architecture in deep network.

Invertibility
\begin{enumerate}
    \item Calibration and \gls{OOD}: \citep{ardizzone_exact_2020}, \citep{nalisnick_hybrid_2019}
    \item Adversarial Robustness:  \citep{jacobsen_excessive_2018}
\end{enumerate}

\subsubsection{Scalable \gls{GP} Methods}
Combination of Laplace approximation and Random Fourier Feature for a non-standard likelihood (integrated log posterior of a Multinomial-Dirichlet model). Formulated as a neural network module amendable to mini-batch update.

\begin{enumerate}
    \item Laplace approximation for multinomial likelihood:
\citep{williams_bayesian_1995}
\citep{rasmussen_gaussian_2006}
\citep{riihimaki_gaussian_2010}
Despite theoretically worse approximation quality for the full posterior \citep{nickisch_approximations_2008}. Strong candidate for neural formulation, tight connection with frequentest training and good computational efficiency.
    \item Random Fourier Feature in deep learning 
    \begin{enumerate}
        \item Frequentest: 
        model \citep{mehrkanoon_deep_2018}
        Theory
        \citep{kawaguchi_deep_2018}. better generalization.
        \item Bayesian (GP). 
        \begin{enumerate}
            \item Prediction: Mostly use \gls{VI} and focus on prediction, e.g.,  Mean-field \gls{VI} \citep{cutajar_random_2017} \citep{hensman_scalable_2015}
    Structured \gls{VI} \citep{hensman_variational_2018}, goals are mostly prediction. inferior approximation for posterior variance. challenge in computation due to complicated optimization landscape.
            \item Uncertainty: Calibration: \citep{tran_calibrating_2019} using  \gls{MCD}.
            \item \gls{OOD}: \citep{domingues_deep_2018}
        \end{enumerate}
    \end{enumerate}

\end{enumerate}

Different Model Formulation
\begin{enumerate}
\item Gamma augmentation: \citep{milios_dirichlet-based_2018}
\item Polya-gamma augmentation: \citep{linderman_dependent_2015}
\end{enumerate}

==> section/section_old/theory_old.tex <==
Comments on Input Distance awareness: \jzl{to convert to full paragraph}
\balaji{you may want to look into enumitem package which allows to control leftmargin indent space}
\begin{itemize}
    % \item A generalization of classic maximum entropy principle for Brier score \citep{grunwald_game_2004}. Application to the context of uncertainty quantification for deep learning is new.
    \item For the purpose of uncertainty quantification, Proposition \ref{thm:minimax} is important in below ways: 
    \begin{itemize}
        \item Theoretic side: The existence of minimax solution (\ref{eq:minimax_solution}) verifies that the learning problem for uncertainty risk minimization (\ref{eq:minimax_loss}) is \textit{sound}, i.e.,  it is well-posed and adopts a unique solution. 
        \item Practical side: Furthermore, it shows that an optimal solution to (\ref{eq:minimax_loss}) not only exists, but also adopts a simple form (\ref{eq:minimax_solution}) which  can be constructed cheaply using the a mixture of the discrete uniform distribution and the in-domain predictive distribution $p(y|\bx, \bx \in \Xsc_{\textup{\texttt{train}}})$ that the model has already learned from data.
        \item Most importantly for \gls{UQ}. It gives a learning-theoretic interpretation to the principle of insufficient reason, which underlies the Bayesian practice of assigning flat priors \citep{murphy_machine_2012, jaynes_probability_2003}.
        It also explains the success of the ensemble approach: distance awareness via diversity \citep{fort_deep_2019}.
        Such design principle was hinted in previous work in uncertainty quantification for deep learning, but was not formalized \citep{malinin_prior_2018}.
    \end{itemize}
    \item  Although the assumption that the domain probability $p^*(\bx \in \Xsc_{\textup{\texttt{train}}})$ is fully known has made Proposition \ref{thm:minimax} somehow theoretical. But it highlighted the fact that a model's ability in characterizing the domain probability $P(\bx \in \Xsc_{\textup{\texttt{train}}})$ is important for reliable uncertainty quantification. Some \gls{OOD} work does this implicitly by training a generative model \citep{nalisnick_deep_2019, ardizzone_exact_2020} or impose adversarial regularization \citep{malinin_prior_2018, lee_training_2018}. In this work, we explore simpler approach by improving the inherent mathematical property of a discriminative neural network. 
    \item In the low-dimensional setting, an ideal model that reflects this principle is the \gls{GP} equipped with a shift-invariant kernel (e.g., a \gls{RBF} kernel). The  posterior uncertainty of a \gls{GP} reflects distance from the training data, and its predictive distribution reverts to prior distribution with high entropy (a softmax Gaussian with high prior variance) at locations that are far from training data \citep{liu_accurate_2019, rasmussen_gaussian_2004}.
    \item Additional comment:
    \begin{itemize}
        \item Proposition \ref{thm:minimax} also covers the case of measuring calibration on the testing dataset. Since strictly speaking testing data are \gls{OOD} in different degree.
        \item It is possible to extend to the case where $P(\bx \in \Xsc_{\texttt{train}})$ is learned, however it requires reasoning about the learning behavior of a particular choice of estimator in recovering the true support of the in-domain distribution \citep{scholkopf_estimating_2001}. leave for future work.
    \end{itemize}
\end{itemize}

Comments on Distance Preservation:\jzl{to convert below to full paragraph}
\begin{itemize}
\item The input distance metric: $||.||_X$ is a suitable metric reflecting semantically meaningful distance in the input space. e.g., not $L_2$ metric in pixel space. Both empirical and theoretical work has shown that the deep learning model are effective in estimating a geometry-preserving metric transform from data manifold $\Xsc$ to the Euclidean space $\Hsc$. \citep{basri_efficient_2016, hauser_principles_2017}. 
\item From a analysis point of view, (\ref{eq:dp}) is  equivalent to the bi-Lipschitz Condition \citep{searcod_metric_2006}. A well-known desirable property: 
\begin{itemize}
    \item Upper bound: prevents over-sensitivity, improve robustness, etc. \citep{anil_sorting_2019}. 
    \item Lower bound: meaningful representation, prevent feature collapse or excessive invariance.\citep{van_amersfoort_simple_2020}.\citep{jacobsen_exploiting_2019}
    \item Near Isometry: Although not stated explicitly, learning a isometric mapping that meaningfully reflects the semantic property in the input space is a common goal in machine learning. For example, image classifiers strive to learn a mapping from image manifold to a space that can be well-separated by a set of linear decision boundaries, and sentences encoders aim to project sentences into a vector space where the cosine distance reflects the semantic similarity in natural language. In practice, it is difficult to guarantee strict isometry without making significant modifications to the existing architecture (e.g., iRevNet), therefore we consider a slightly weaker condition, i.e., Bi-Lipschitz. \citep{perrault-joncas_metric_2017}.
\end{itemize}
\item  \balaji{we may want to move this to discussion} Distance Preservation is not guanrantee in general (adversarial examples \citep{jacobsen_excessive_2018}, unscaled inner product distance to decision boundary Figure \ref{fig:2d_exp_oval_deepens} and \ref{fig:2d_exp_moon_deepens}). 
The lack of distance awareness in deep learning is also made evident by the study of adversarial examples, which show that a typical deep model can not only be  sensitive in semantically-meaningless perturbations in the input space, and also at times be invariant to semantically-meaningful perturbations \citep{jacobsen_excessive_2018, jacobsen_exploiting_2019}. 
\end{itemize}


==> section/tables/cifar.tex <==
\begin{table*}[th]
\centering
%\scalebox{0.7}{
\resizebox{1.\textwidth}{!}{%
\Large
\begin{tabular}{c||cc|c|cc|c||cc|c|cc|c}
\toprule
& \multicolumn{6}{c||}{CIFAR-10} & 
\multicolumn{6}{c}{CIFAR-100}
\\
\midrule
& 
\multicolumn{1}{c}{ } & 
\multicolumn{1}{c}{ } &
\multicolumn{1}{c}{Corrupted} &
\multicolumn{2}{c}{OOD AUPR ($\uparrow$)} &
Latency &
\multicolumn{1}{c}{ } & 
\multicolumn{1}{c}{ } &
\multicolumn{1}{c}{Corrupted} &
\multicolumn{2}{c}{OOD AUPR ($\uparrow$)} &
Latency
\\
Method  & 
Acc ($\uparrow$) & ECE ($\downarrow$) & Acc/ECE & 
SVHN & CIFAR-100 & {(ms)} &
Acc ($\uparrow$) & ECE ($\downarrow$) & Acc/ECE & 
SVHN & CIFAR-10 & {(ms)} 
\\
\midrule
Deterministic & 96.0 & 0.023 & 72.9  / 0.153 & 0.7810 & 0.8352 & \textbf{3.91} & 79.8  & 0.085 & 50.5 / 0.239 & 0.8824 & 0.7452 & \textbf{5.20}
\\
\midrule
\glsunset{MCDGP}\gls{MCDGP} & 95.5 & 0.024 & 70.0  / 0.100 & 0.9599 & 0.8631 & 29.53 & 79.5 & 0.085 & 45.0 / 0.159 & 0.8732 & 0.7536 & 
44.20 \\
\glsunset{DUQ}\gls{DUQ}  & 94.7 & 0.034 & 71.6 / 0.183 & 0.9733 & 0.8537 & 8.68 & 78.5 & 0.119 & 50.4 / 0.281 & 0.8780 & 0.7321 & 
6.51\\
\midrule
\glsunset{MCD}\gls{MCD} & 96.0 & 0.024 & 70.0  / 0.116 & 0.9714 & 0.8320 & 27.10 & 79.6 & 0.050 & 42.6 / 0.202 & 0.8320 & 0.7568 & 
46.79\\
Deep Ensembles & \textbf{96.6} & \textbf{0.010} & \textbf{77.9} / \textbf{0.087} & 0.9640 & 0.8875 & 38.10 & \textbf{80.2} & \textbf{0.021} & \textbf{54.1} / 0.138 & 0.8875 & 0.7796 & 42.06\\
\midrule
\gls{SNGP} (Ours) & 95.9 & 0.018 & 74.6  / 0.090 & \textbf{0.9901} & \textbf{0.9050} & 6.25 & 79.9 & 0.025 & 49.0 / \textbf{0.117} & \textbf{0.9233} & \textbf{0.8013} & 6.94\\
\bottomrule
\end{tabular}
}
\caption{\small{
Results for WRN-28-10 on CIFAR-10/100
%CIFAR-1/-100, 
averaged over 10 seeds. More details in Appendix \ref{sec:result_app}.
\balaji{would be replaced with detail results}
}} 
\vspace{-1em}
\label{tb:cifar}
\end{table*}

==> section/tables/clinc.tex <==
\begin{table}[h!]
\centering
\scalebox{0.7}{ % NeurIPS
%\resizebox{1.\columnwidth}{!}{% ICML
\begin{tabular}{cc|c|cc|c}
\toprule
& \multicolumn{1}{c}{Accuracy ($\uparrow$)} & 
\multicolumn{1}{c}{ECE ($\downarrow$)} &
\multicolumn{2}{c}{OOD} & Latency \\
Method  &   &   & 
AUROC ($\uparrow$) & AUPR ($\uparrow$) & 
{\small (ms / example)}\\
\midrule
Deterministic & 96.5 & 0.0236 & 0.8970 & 0.7573 & \textbf{10.42} \\
\midrule
\gls{MCDGP} & 95.9 & 0.0146 & 0.9055 & 0.8030 & 88.38\\
\gls{DUQ} & 96.0 & 0.0585 & 0.9173 & 0.8058 & 15.60\\
\midrule
\gls{MCD} & 96.5 & 0.0210  & 0.9382 & 0.7997 & 85.62 \\
Deep Ensemble & \textbf{97.5} & 0.0128  & 0.9635 & 0.8616 & 84.46 \\
\midrule
\gls{SNGP} & 96.6 & \textbf{0.0115} & \textbf{0.9688} & \textbf{0.8802} & 17.36 \\
\bottomrule
\end{tabular}
}
\caption{\small{
Results for BERT$_{\texttt{Base}}$ on CLINC \gls{OOS}, averaged over 10 seeds. More details in Appendix \ref{sec:result_app}.
\balaji{would be replaced with detail results}
%\balaji{maybe add memory/parameter complexity of models as well?}
}}
\vspace{-1em}
\label{tb:clinc}
\end{table}

